The intersection homology D--module in finite characteristic

Let R be a regular, local and F-finite ring defined over a field of finite characteristic. Let I be an ideal of height c with normal quotient $A=R/I$. It is shown that the local cohomology module H^c_I(R) contains a unique simple D_R--submodule L(A,R). This should be viewed as a finite characteristic analog of the Kashiwara--Brylinski D_R--module in characteristic zero which corresponds to the intersection cohomology complex via the Riemann--Hilbert correspondence. Besides the existence of L(A,R), more importantly, we give its construction as a certain dual of the tight closure of zero in $H^d_m(A)$. We obtain a precise D_R--simplicity criterion for H^c_I(R), namely H^c_I(R) is D_R--simple if and only if the tight closure of zero in H^d_m(A) is Frobenius nilpotent, in particular this is the case if A is F--rational. Furthermore, the techniques developed imply a result in tight closure theory, saying that the parameter test module commutes with completion.

==> parts/abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                          %%
%%   This is file: abstract.tex                             %%
%%   It contains the Abstract of my                         %%
%%   dissertation: dissertation.tex                         %%
%%                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Let $R$ be a regular, local and $F$--finite ring defined over a field of
finite characteristic. Let $I$ be an ideal of height $c$ such that the
completion of the quotient $A=R/I$ is a domain. It is shown that the local
cohomology module $H^c_I(R)$ contains a unique simple $D_R$--submodule
$\Ll(A,R)$. This should be viewed as an analog of the Kashiwara--Brylinski
$D_R$--module in characteristic zero which corresponds to the intersection
cohomology complex via the Riemann--Hilbert correspondence. Besides the
existence of $\Ll(A,R)$, more importantly, we give a concrete construction
as a certain dual of the tight closure of zero in $H^d_m(A)$.

In order to prove this result the theory of $R[F^\infty]$--modules and
techniques from the theory of tight closure play a crucial role. A key
result tying $R[F^\infty]$--modules to $D_R$--modules is that if $k$ is an
uncountable algebraically closed field then a finitely generated simple
unit $R[F^\infty]$ is simple as a $D_R$--module. The given construction of
$\Ll(A,R)$ yields a precise $D_R$--simplicity criterion for $H^c_I(R)$,
namely $H^c_I(R)$ is $D_R$--simple if and only if the tight closure of
zero in $H^d_m(A)$ is Frobenius nilpotent, in particular this is the case
if $A$ is $F$--rational.

Furthermore, the techniques developed imply a result in tight closure
theory, saying that the parameter test module commutes with completion.


==> parts/gabstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                          %%
%%   This is file: gabstract.tex                            %%
%%   It contains the German Abstract of my                  %%
%%   dissertation: dissertation.tex                         %%
%%                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\selectlanguage{german}



Sei $R$ ein regul"arer, lokaler Ring "uber einem K"orper endlicher
Charakteristik. Sei $I$ ein ideal von $R$ der H"ohe $c$, so das der
Quotient $A=R/I$ analytisch irreduziebel ist. Es wird gezeigt dass der
lokale Kohomologiemodul $H^c_I(R)$ einen eindeutigen einfachen
$D_R$--Untermodul $\Ll(A,R)$ besitzt. Dieser kann als das Gegenst"uck des
Kashiwara--Brylinskischen $D_R$--moduls in Charakteristik Null angesehen
werden, welchesr durch die Riemann--Hilbert Korrespondenz mit dem
Intersection Homologie complex identifiziert ist.

Beim Beweis dieses Resultas spielen die Theorie der $R[F^\infty]$--Moduln
und Methoden aus der Tight Closure Theory eine wichtige Rolle. Ein
ausschlaggebendes Resultat, welches den Zusammenhang zwischen
$F[R^\infty]$ und $D_R$--Modul kn"upft, besagt dass ein einfacher
$R[F^\infty]$--Modul als $D_R$--Modul ebenfalls einfach ist, angenommen
dass $R$ einen "uberabz"ahlbaren algebraisch abgeschlossenen K"orper enth"alt.
Die Konstruktion von $\Ll(A,R)$ impliziert ein Kriterium f"ur die
Einfachheit von $H^c_I(R)$ als $D_R$--modul; n"amlich, $H^c_I(R)$ is
$D_R$--einfach genau dann wenn die tight closure von Null in $H^d_m(A)$
Frobenius nilpotent ist. Insbesondere ist $H^c_I(R)$ immer $D_R$--einfach
wenn $A$ $F$--rational ist.

\selectlanguage{english}

